Incorporating Geo-Diverse Knowledge into Prompting for Increased Geographical Robustness in Object Recognition

Existing object recognition models have been shown to lack robustness in diverse geographical scenarios due to domain shifts in design and context. Class representations need to be adapted to more accurately reflect an object concept under these shifts. In the absence of training data from target geographies, we hypothesize that geographically diverse descriptive knowledge of categories can enhance robustness. For this purpose, we explore the feasibility of probing a large language model for geography-based object knowledge, and we examine the effects of integrating knowledge into zero-shot and learnable soft prompting with CLIP. Within this exploration, we propose geography knowledge regularization to ensure that soft prompts trained on a source set of geographies generalize to an unseen target set. Accuracy gains over prompting baselines on DollarStreet while training only on Europe data are up to +2.8/1.2/1.6 on target data from Africa/Asia/Americas, and +4.6 overall on the hardest classes. Competitive performance is shown vs. few-shot target training, and analysis is provided to direct future study of geographical robustness.

==> figures/geonet_few_shot_tgt.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.19]
    {images/geonet_tgt_few-shot.png}
    \caption{\textbf{Country knowledge-regularized soft prompts trained on source data (USA) vs. few-shot soft prompts trained on target data (Asia ), GeoNet}. }
    \label{few_shot_tgt_fig}
\end{figure}

==> figures/supp_top5_bottom5_histogram_dollarstreet.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.5]  % Adjust the scale as needed
    {images/top5_bottom_5_dollarstreet_supp.png}
    \vspace{-3mm}
    \caption{\textbf{Class-wise comparison of Ours vs. CoOp on Dollarstreet.} We sort the top 25 most frequent categories based on $\Delta = Acc(Ours) - Acc(CoOp)$ and show the bottom 5 and top 5 categories. Leveraging LLM descriptors can be most useful on objects that may have country-specific characteristics, while it may hurt the performance on more generic objects such as \textit{airliner} as it produces fine-grained descriptors like \textit{having two engines} which may not be visible in the image.}
    \label{supp:top5_bottom5_geonet}
\end{figure*}


==> figures/supp_top5_bottom5_histogram_geonet.tex <==
\begin{figure}[!tp]
    \centering
    \includegraphics[scale=0.5]  % Adjust the scale as needed
    {images/top5_bottom_5_geonet_supp.png}
    \vspace{-3mm}
    \caption{\textbf{Class-wise comparison of Ours vs. CoOp on GeoNet.} We sort the top 25 most frequent categories based on $\Delta = Acc(Ours) - Acc(CoOp)$ and show the bottom 5 and top 5 categories. Leveraging LLM descriptors can be most useful on objects that may have country-specific characteristics, while it may hurt the performance on more generic objects such as \textit{airliner} as it produces fine-grained descriptors like \textit{having two engines} which may not be visible in the image.}
    \label{supp:top5_bottom5_geonet}
\end{figure
}


==> tables/all_src_tgt_reg.tex <==
    
\begin{table}
    \begin{center}
    \begin{tabular}{c|c|c|ccc|}
    \hline
     Countries  &  LLM &  In   & Source & Target  \\
    
  in Ensemble &  Desc &  Country  & Acc &  Acc  \\
    
    \hline\hline
    Source & & \checkmark &  72.5 &  62.8 \\
    \hline
    Target & & \checkmark &  71.8 &  63.5  \\
    \hline
    All & & \checkmark &  72.8 &  63.2 \\
    \hline\hline
    Source & \checkmark &  &  73.0 &  63.4  \\
    \hline
    Target & \checkmark &  &  73.2 &  63.2  \\
    \hline
    All & \checkmark &  &  72.3 & 63.4 \\
    \hline
    \hline
    Source & \checkmark & \checkmark & 73.5  &  63.1  \\
    \hline
    Target & \checkmark & \checkmark & \textbf{73.6} &  \textbf{64.0}  \\
    \hline
    All & \checkmark & \checkmark & 72.6 &  63.8 \\
    \hline
    \end{tabular}
    \end{center}
    \caption{Comparing regularization results using different country ensemble sets and prompt formats. ViT }
    \label{tabel:all_src_tgt_reg}
\end{table}

==> tables/bacc_and_oacc_soft_prompts.tex <==
 \setlength{\tabcolsep}{0.4pt}

\begin{table*}[t]

    \begin{center}
        \renewcommand{\arraystretch}{0.8}

    \begin{tabular}{c|c|cccc|cccc|cccc|cccc|cccc}
        \hline
         && \multicolumn{4}{c|}{\textit{\small\textbf{Source}}} 
         & \multicolumn{16}{c}{\textit{\small\textbf{Target}}}  \\
        
         \small \textbf{Encoder} & \small \textbf{Prompting Method} & \multicolumn{4}{c|}{\small\textbf{Europe}} &\multicolumn{4}{c}{\small\textbf{Africa}} & \multicolumn{4}{c}{\small\textbf{Asia}} & \multicolumn{4}{c}{\small\textbf{Americas}} & \multicolumn{4}{c}{\small\textbf{Total}} \\
        
         & & \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} & \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c|}{\small $\Delta$} &  \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$}  &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$}   \\
    
    \hline\hline
    
        \rowcolor{LLGray}\cellcolor{white} \small ViT-B/16 &
        
          \small CoOp \cite{zhou2022learning} 
        % Europe
         & \small 72.2 & \scriptsize - & \small 73.3 & \scriptsize -
         % Africa
         & \small 53.9 & \scriptsize - & \small 48.5 & \scriptsize - 
         % Asia
         & \small 61.5 & \scriptsize - & \small 60.7 & \scriptsize -
         % Americas
         & \small 68.6 & \scriptsize - & \small 67.8 & \scriptsize -
         % Total
         & \small 61.7 & \scriptsize - & \small 59.7 & \scriptsize - \\
         
         \rowcolor{LLGray} \cellcolor{white} & \small CoCoOp \cite{Zhou_2022_CVPR} 
         & \small 73.2 & \scriptsize - & \small \textbf{74.4} & \scriptsize -
          & \small 54.3 & \scriptsize - & \small 48.4 & \scriptsize -
         & \small 61.2 & \scriptsize - & \small 60.6 & \scriptsize -
         & \small 68.3 & \scriptsize - & \small 67.1 & \scriptsize -
         & \small 61.4 & \scriptsize - & \small 59.5 & \scriptsize - \\
         
         \rowcolor{LLGray} \cellcolor{white} & \small KgCoOp ($\lambda$=8) \cite{yao2023visual} 
         & \small 72.6 & \scriptsize - & \small 73.6 & \scriptsize -
         & \small 54.1 & \scriptsize - & \small 48.2 & \scriptsize - 
         & \small 61.5 & \scriptsize - & \small 60.7 & \scriptsize -
         & \small 68.3 & \scriptsize - & \small 67.0 & \scriptsize -
         & \small 61.6 & \scriptsize - & \small 59.5 & \scriptsize - \\
        
         \rowcolor{LLGray} \cellcolor{white} & \small KgCoOp ($\lambda$=4) \cite{yao2023visual} 
         & \small 73.1 & \scriptsize - & \small 73.9 & \scriptsize -
         & \small 54.4 & \scriptsize - & \small 49.5 & \scriptsize -   
         & \small 62.6 & \scriptsize - & \small 62.1 & \scriptsize - 
         & \small 68.7 & \scriptsize - & \small 68.0 & \scriptsize -
         & \small 62.4 & \scriptsize - & \small 60.7 & \scriptsize-  \\
         
         & \small CountryInPrompt Reg 
         & \small 71.8 & \scriptsize \color{red}{-1.4} & \small 73.4 & \scriptsize \color{red}{-1.0}
         & \small 56.8 & \scriptsize \color{Greenish}{+2.4}  & \small \textbf{52.0} & \scriptsize \color{Greenish}{+2.5} 
         & \small 63.0 & \scriptsize \color{Greenish}{+0.4} & \small \textbf{63.6} & \scriptsize \color{Greenish}{+1.5} 
         & \small 69.8 & \scriptsize \color{Greenish}{+1.1} & \small 68.8 & \scriptsize \color{Greenish}{+0.8}
         & \small 63.5 & \scriptsize \color{Greenish}{+1.1} & \small \textbf{62.3} & \scriptsize \color{Greenish}{+1.6} \\
         
         & \small CountryLLM Reg 
         & \small 73.2 & \scriptsize \color{black}{0.0} & \small 73.9 & \scriptsize \color{red}{-0.5}
         & \small 55.6 & \scriptsize \color{Greenish}{+1.2} & \small 50.6 & \scriptsize \color{Greenish}{+1.1} 
         & \small 63.0 & \scriptsize \color{Greenish}{+0.4} & \small 62.8 & \scriptsize \color{Greenish}{+0.7}
         & \small 70.0 & \scriptsize \color{Greenish}{+1.3} & \small \textbf{69.1} & \scriptsize \color{Greenish}{+1.1}
         & \small 63.2 & \scriptsize \color{Greenish}{+0.8} & \small 61.6 & \scriptsize \color{Greenish}{+0.9} \\
         
         & \small CountryInPrompt+LLM Reg  
         & \small \textbf{73.6} & \scriptsize \color{Greenish}{+0.4} & \small 74.0 & \scriptsize \color{red}{-0.4}
         & \small \textbf{57.2} & \scriptsize \color{Greenish}{+2.8} & \small 51.9 & \scriptsize \color{Greenish}{+2.4} 
         & \small \textbf{63.8} & \scriptsize \color{Greenish}{+1.2} & \small 63.4 & \scriptsize \color{Greenish}{+1.3} 
         & \small \textbf{70.3} & \scriptsize \color{Greenish}{+1.6} & \small 68.8 & \scriptsize \color{Greenish}{+0.8}
         & \small \textbf{64.0} & \scriptsize \color{Greenish}{+1.6} & \small 62.2 & \scriptsize \color{Greenish}{+1.5} \\
         
    \hline\hline
        
        \rowcolor{LLGray} \cellcolor{white} \small RN50 
        
        & \small CoOp \cite{zhou2022learning} 
        & \small 64.6 & \scriptsize - & \small 65.9 & \scriptsize -
        & \small 45.2 & \scriptsize - & \small 40.3 & \scriptsize - 
        & \small 51.6 & \scriptsize - & \small 51.3 & \scriptsize - 
        & \small 59.5 & \scriptsize - & \small 58.5 & \scriptsize -
        & \small 52.2 & \scriptsize - & \small 50.6 & \scriptsize -\\
        
        \rowcolor{LLGray} \cellcolor{white} & \small CoCoOp \cite{Zhou_2022_CVPR} 
        & \small 62.9 & \scriptsize - & \small 64.1 & \scriptsize -
        & \small 44.5 & \scriptsize - & \small 39.1 & \scriptsize - 
        & \small 51.0 & \scriptsize - & \small 50.3 & \scriptsize - 
        & \small 58.3 & \scriptsize - & \small 57.7 & \scriptsize -
        & \small 51.4 & \scriptsize - & \small 49.6 & \scriptsize - \\
        
        \rowcolor{LLGray} \cellcolor{white}  & \small KgCoOp ($\lambda$=8) \cite{yao2023visual} 
        & \small 61.6 & \scriptsize - & \small 64.6 & \scriptsize -
        & \small 45.2 & \scriptsize - & \small 41.7 & \scriptsize -
        & \small 52.6 & \scriptsize - & \small 52.8 & \scriptsize - 
        & \small 59.6 & \scriptsize - & \small 58.8 & \scriptsize -
        & \small 52.8 & \scriptsize - & \small 51.8 & \scriptsize -  \\
        
        \rowcolor{LLGray} \cellcolor{white}  & \small KgCoOp ($\lambda$=4) \cite{yao2023visual} 
        & \small 63.5 & \scriptsize - & \small 65.0 & \scriptsize -
        & \small 46.3 &\scriptsize - & \small 42.2 & \scriptsize - 
        & \small 53.9 & \scriptsize - & \small 53.4 & \scriptsize - 
        & \small \textbf{60.5} & \scriptsize - & \small 59.5 & \scriptsize -
        & \small 53.9 & \scriptsize - & \small 52.4 & \scriptsize - \\
        
        & \small CountryInPrompt Reg 
        & \small 63.5 & \scriptsize \color{red}{-1.1} & \small 64.9 & \scriptsize \color{red}{-1.0}
        & \small 48.0 & \scriptsize \color{Greenish}{+1.7} & \small 42.9 & \scriptsize \color{Greenish}{+0.7}
        & \small 53.9 & \scriptsize \color{black}{0.0} & \small 53.9 & \scriptsize \color{Greenish}{+0.5}
        & \small 60.3 & \scriptsize \color{red}{-0.2} & \small 59.3 & \scriptsize \color{red}{-0.2}
        & \small 54.3 & \scriptsize \color{Greenish}{+0.4} & \small 52.8 & \scriptsize \color{Greenish}{+0.4}  \\
        
         & \small CountryLLM Reg 
         & \small 64.5 & \scriptsize \color{red}{-0.1} & \small 65.5 & \scriptsize \color{red}{-0.4}
         & \small 47.4 & \scriptsize \color{Greenish}{+1.1} & \small 41.7 & \scriptsize \color{red}{-0.5} 
         & \small 54.2 & \scriptsize \color{Greenish}{+0.3} & \small 53.3 & \scriptsize \color{red}{-0.1}
         & \small 59.9 & \scriptsize \color{red}{-0.6} & \small 59.2 & \scriptsize  \color{red}{-0.3}
         & \small 54.3 & \scriptsize \color{Greenish}{+0.4} & \small 52.2 & \scriptsize \color{red}{-0.2} \\
         
         & \small CountryInPrompt+LLM Reg    
         & \small \textbf{65.5} & \scriptsize \color{Greenish}{+0.9} & \small \textbf{66.8} & \scriptsize \color{Greenish}{+0.9}
         & \small \textbf{48.1} & \scriptsize \color{Greenish}{+1.8} & \small \textbf{43.1} & \scriptsize \color{Greenish}{+0.9} 
         & \small \textbf{54.5} & \scriptsize \color{Greenish}{+0.6} & \small \textbf{54.0} & \scriptsize \color{Greenish}{+0.6}
         & \small 60.4 & \scriptsize \color{red}{-0.1} & \small \textbf{59.6} & \scriptsize\color{Greenish}{+0.1}
         & \small \textbf{54.8} & \scriptsize \color{Greenish}{+0.9} & \small \textbf{53.0} & \scriptsize \color{Greenish}{+0.6} \\

    \hline
    \end{tabular}
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Evaluating country knowledge-regularized soft prompts, top1 balanced accuracy (BAcc) and overall accuracy (OAcc) on DollarStreet.} We emphasize that our regularization aims to improve \textbf{target} performance on unseen geographies, rather than source. We compare regularizing prompts with country names (CountryInPrompt), country-specific LLM knowledge (CountryLLM), and both (CountryInPrompt+LLM), with gains(\color{Greenish}{green}\color{black})/drops(\color{red}{red}\color{black}) shown vs. the \textit{best} of various soft prompt baselines. Our CountryInPrompt+LLM achieves notable gains in target, especially on Africa. We use regularization weight $\lambda$=4, so we compare to KgCoOp at $\lambda$=8 (default) and $\lambda$=4. Each method uses 16 shots \& context length 4.}
    \label{table:soft_prompt}
\end{table*}

==> tables/bacc_and_oacc_zeroshot.tex <==
 \setlength{\tabcolsep}{0.5pt}

\begin{table*}[t]

    \begin{center}
    \renewcommand{\arraystretch}{0.8}

    \begin{tabular}{c|c|cccc|cccc|cccc|cccc|cccc}
        \hline
        \textbf{\small Encoder} & \textbf{\small Prompting Method} & \multicolumn{4}{c}
        {\textbf{\small Europe}} & \multicolumn{4}{c}{\textbf{\small Africa}} &\multicolumn{4}{c}{\textbf{\small Asia}} & \multicolumn{4}{c}{\textbf{\small Americas}} & \multicolumn{4}{c}{\textbf{\small Total}} \\
         & &  \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$} & \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$} & \multicolumn{1}{c}{\small BAcc} & \multicolumn{1}{c}{\small $\Delta$} &  \multicolumn{1}{c}{\small OAcc} & \multicolumn{1}{c}{\small $\Delta$}
         
         \\
    \hline\hline \rowcolor{LLGray}
        \small \cellcolor{white} ViT-B/32  
        & \small Zero-Shot CLIP \cite{radford2021learning} 
        & \small 59.1 & \scriptsize - 
        & \small 56.3 & \scriptsize - 
        & \small 43.7 & \scriptsize - 
        & \small 38.3 & \scriptsize - 
        & \small 50.8 & \scriptsize - 
        & \small 47.4 & \scriptsize - 
        & \small \textbf{55.3} & \scriptsize - 
        & \small 53.1 & \scriptsize - 

        & \small 51.7 & \scriptsize -
        & \small 48.3 & \scriptsize -\\
        
         \rowcolor{LLGray}
        \small \cellcolor{white} & \small GeneralLLM \cite{menon2022visual}
         & \small 57.3 & \scriptsize \color{red}{-1.8} 
         & \small 55.4 & \scriptsize \color{red}{-0.9} 
         & \small 44.3 & \scriptsize \color{Greenish}{+0.6} 
         & \small 38.4 & \scriptsize \color{Greenish}{+0.1} 
         & \small 50.9 & \scriptsize \color{Greenish}{+0.1} 
         & \small 48.2 & \scriptsize \color{Greenish}{+0.8} 
         & \small 54.6 & \scriptsize \color{red}{-0.7} 
         & \small 52.2 & \scriptsize \color{red}{-0.9} 

         & \small 51.4 & \scriptsize \color{red}{-0.3}
         & \small 48.4 & \scriptsize \color{Greenish}{+0.1}  \\

         & \small CountryInPrompt 

         & \small 57.5 & \scriptsize \color{red}{-1.6} 
         & \small 55.2 & \scriptsize \color{red}{-1.1} 
         & \small 45.2 & \scriptsize \color{Greenish}{+1.5} 
         & \small 41.0 & \scriptsize \color{Greenish}{+2.7} 
         & \small 51.9 & \scriptsize \color{Greenish}{+1.1} 
         & \small 49.7 & \scriptsize \color{Greenish}{+2.3} 
         & \small 55.0 & \scriptsize \color{red}{-0.3} 
         & \small 52.3 & \scriptsize \color{red}{-0.8} 

         & \small 52.1 & \scriptsize \color{Greenish}{+0.4}
         & \small 49.5 & \scriptsize \color{Greenish}{+1.2} \\
         
         & \small CountryLLM 
         & \small 59.4 & \scriptsize \color{Greenish}{+0.3} 
         & \small \textbf{57.5} & \scriptsize \color{Greenish}{+1.2} 
         & \small 45.2 & \scriptsize \color{Greenish}{+1.5} 
         & \small 40.7 & \scriptsize \color{Greenish}{+2.4} 
         & \small 52.1 & \scriptsize \color{Greenish}{+1.3} 
         & \small 49.6 & \scriptsize \color{Greenish}{+2.2} 
         & \small \textbf{55.3} & \scriptsize \color{black}{0.0} 
         & \small \textbf{53.4} & \scriptsize \color{Greenish}{+0.3} 

         & \small 52.6 & \scriptsize \color{Greenish}{+0.9}
         & \small 50.0 & \scriptsize \color{Greenish}{+1.7} \\
         

         
         &  \small CountryInPrompt+LLM  
          & \small \textbf{60.8} & \scriptsize \color{Greenish}{+1.7}
         & \small \textbf{57.5} & \scriptsize \color{Greenish}{+1.2} 
         & \small \textbf{45.3} & \scriptsize \color{Greenish}{+1.6} 
         & \small \textbf{41.3} & \scriptsize \color{Greenish}{+3.0} 
         & \small \textbf{52.2} & \scriptsize \color{Greenish}{+1.4}
         & \small \textbf{50.1} & \scriptsize \color{Greenish}{+2.7}
         & \small 55.0 & \scriptsize \color{red}{-0.3} 
         & \small 52.9 & \scriptsize \color{red}{-0.2} 

         & \small \textbf{52.8} & \scriptsize \color{Greenish}{+1.1}
         & \small \textbf{50.3} & \scriptsize \color{Greenish}{+2.0}\\
         
    \hline\hline \rowcolor{LLGray}
       \small  \cellcolor{white}ViT-B/16  & \small Zero-Shot CLIP \cite{radford2021learning}  
        & \small 64.3 & \scriptsize - 
       & \small 61.5 & \scriptsize - 
       & \small 46.9 & \scriptsize - 
       & \small 42.9 & \scriptsize - 
       & \small 53.9 & \scriptsize - 
       & \small 52.7 & \scriptsize - 
       & \small \textbf{60.1} & \scriptsize - 
       & \small 58.0 & \scriptsize - 
       & \small 55.5 & \scriptsize - 
       & \small 53.4 & \scriptsize - \\
       
         \rowcolor{LLGray}
        \small \cellcolor{white} & \small GeneralLLM \cite{menon2022visual} 
          & \small 64.2 & \scriptsize \color{red}{-0.1} 
         & \small 61.4 & \scriptsize \color{red}{-0.1} 
         & \small 48.8 & \scriptsize \color{Greenish}{+1.9} 
         & \small 44.9 & \scriptsize \color{Greenish}{+2.0} 
         & \small \textbf{56.0} & \scriptsize \color{Greenish}{+2.1} 
         & \small 55.0 & \scriptsize \color{Greenish}{+2.3} 
         & \small 58.5 & \scriptsize \color{red}{-1.6} 
         & \small 56.9 & \scriptsize \color{red}{-1.1} 

         & \small 56.8 & \scriptsize \color{Greenish}{+1.3}
         & \small 54.6 & \scriptsize \color{Greenish}{+1.2} \\

         
         & \small CountryInPrompt 
         & \small 63.9 & \scriptsize \color{red}{-0.4} 
         & \small 61.5 & \scriptsize \color{black}{0.0} 
         & \small 49.6 & \scriptsize \color{Greenish}{+2.7} 
         & \small 46.2 & \scriptsize \color{Greenish}{+3.3} 
         & \small 55.7 & \scriptsize \color{Greenish}{+1.8} 
         & \small 54.8 & \scriptsize \color{Greenish}{+2.1} 
         & \small 59.3 & \scriptsize \color{red}{-0.8} 
         & \small 57.1 & \scriptsize \color{red}{-0.9} 

         & \small 56.6 & \scriptsize \color{Greenish}{+1.1}
         & \small 54.8 & \scriptsize \color{Greenish}{+1.4}\\

         & \small CountryLLM  
         & \small 65.2 & \scriptsize \color{Greenish}{+0.9} 
         & \small \textbf{62.9} & \scriptsize \color{Greenish}{+1.4} 
         & \small 49.6 & \scriptsize \color{Greenish}{+2.7} 
         & \small 45.4 & \scriptsize \color{Greenish}{+2.5} 
         & \small 55.6 & \scriptsize \color{Greenish}{+1.7} 
         & \small 54.9 & \scriptsize \color{Greenish}{+2.2} 
         & \small 59.7 & \scriptsize \color{red}{-0.4} 
         & \small \textbf{58.4} & \scriptsize \color{Greenish}{+0.4} 

         & \small 57.0 & \scriptsize \color{Greenish}{+1.5}
         & \small 55.1 & \scriptsize \color{Greenish}{+1.7} \\
         
         & \small CountryInPrompt+LLM 
         & \small \textbf{65.5} & \scriptsize \color{Greenish}{+1.2} 
         & \small 62.6 & \scriptsize \color{Greenish}{+1.1} 
         & \small \textbf{50.8} & \scriptsize \color{Greenish}{+3.9} 
         & \small \textbf{47.1} & \scriptsize \color{Greenish}{+4.2} 
         & \small \textbf{56.0} & \scriptsize \color{Greenish}{+2.1} 
         & \small \textbf{55.7} & \scriptsize \color{Greenish}{+3.0} 
         & \small 59.7 & \scriptsize \color{red}{-0.4} 
         & \small 58.2 & \scriptsize \color{Greenish}{+0.2} 
         & \small \textbf{57.4} & \scriptsize \color{Greenish}{+1.9}
         & \small \textbf{55.8} & \scriptsize \color{Greenish}{+2.4}\\
    \hline
    \hline
    \rowcolor{LLGray}
        \small \cellcolor{white} RN50 
        & \small Zero-Shot CLIP \cite{radford2021learning} 
        & \small 53.0 & \scriptsize - 
        & \small 51.8 & \scriptsize - 
        & \small 38.0 & \scriptsize - 
        & \small 34.4 &  \scriptsize - 
        & \small 44.4 & \scriptsize - 
        & \small 44.0 & \scriptsize - 
        & \small 49.8 & \scriptsize - 
        & \small 47.3 & \scriptsize - 

        & \small 45.7 & \scriptsize -
        & \small 44.2 & \scriptsize -  \\
        

         \rowcolor{LLGray}
        \small \cellcolor{white} & \small GeneralLLM \cite{menon2022visual}
         & \small 55.5 & \scriptsize \color{Greenish}{+2.5} 
         & \small 53.2 & \scriptsize \color{Greenish}{+1.4} 
         & \small 40.9 & \scriptsize \color{Greenish}{+2.9} 
         & \small 36.0 & \scriptsize \color{Greenish}{+1.6} 
         & \small 46.9 & \scriptsize \color{Greenish}{+2.5} 
         & \small 45.0 & \scriptsize \color{Greenish}{+1.0} 
         & \small 50.3 & \scriptsize \color{Greenish}{+0.4} 
         & \small 48.3 & \scriptsize \color{Greenish}{+1.0}

         & \small 47.9 & \scriptsize \color{Greenish}{+2.2}
         & \small 45.4 & \scriptsize \color{Greenish}{+1.2}   \\
         

         
         & \small CountryInPrompt 

         & \small 54.5 & \scriptsize \color{Greenish}{+1.5} 
         & \small 52.2 & \scriptsize \color{Greenish}{+0.4} 
         & \small \textbf{43.4} & \scriptsize \color{Greenish}{+5.4} 
         & \small 38.7 & \scriptsize \color{Greenish}{+4.3} 
         & \small 47.0 & \scriptsize \color{Greenish}{+2.6} 
         & \small 45.4 & \scriptsize \color{Greenish}{+1.4}
         & \small 50.8 & \scriptsize \color{Greenish}{+1.0} 
         & \small 48.5 & \scriptsize \color{Greenish}{+1.2} 

         & \small 48.4 & \scriptsize \color{Greenish}{+2.7}
         & \small 45.9 & \scriptsize \color{Greenish}{+1.7}   \\

         & \small CountryLLM 
         & \small 56.2 & \scriptsize \color{Greenish}{+3.2}
         & \small 54.1 & \scriptsize \color{Greenish}{+2.3} 
         & \small 41.1 & \scriptsize \color{Greenish}{+3.1} 
         & \small 36.9 & \scriptsize \color{Greenish}{+2.5} 
         & \small 47.3 & \scriptsize \color{Greenish}{+2.9} 
         & \small 45.7 & \scriptsize \color{Greenish}{+1.7} 
         & \small 50.4 & \scriptsize \color{Greenish}{+0.6} 
         & \small 48.7 & \scriptsize \color{Greenish}{+1.4} 

         & \small 48.3 & \scriptsize \color{Greenish}{+2.6}
         & \small 46.1 & \scriptsize \color{Greenish}{+1.9} \\
         
         & \small CountryInPrompt+LLM 
         & \small \textbf{56.4} & \scriptsize \color{Greenish}{+3.4}
         & \small \textbf{54.7} & \scriptsize \color{Greenish}{+2.9} 
         & \small 43.0 & \scriptsize \color{Greenish}{+5.0} 
         & \small \textbf{38.9} & \scriptsize \color{Greenish}{+4.5}
         & \small \textbf{48.0} & \scriptsize \color{Greenish}{+3.6} 
         & \small \textbf{47.1} & \scriptsize \color{Greenish}{+3.1} 
         & \small \textbf{50.9} & \scriptsize \color{Greenish}{+1.1} 
         & \small \textbf{49.6}  & \scriptsize \color{Greenish}{+2.3} 

         & \small \textbf{49.1} & \scriptsize \color{Greenish}{+3.4}
         & \small \textbf{47.3} & \scriptsize \color{Greenish}{+3.1}\\ 
    \hline
    \end{tabular}
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Zero-shot CLIP with descriptive knowledge prompts, top1 balanced accuracy (BAcc) and overall accuracy (OAcc) on DollarStreet.} We test the methodology from \cite{menon2022visual}, our country-specific LLM probing (CountryLLM), adding country names to prompts (CountryInPrompt), and both country strategies combined (CountryInPrompt+LLM), with gains(\color{Greenish}{green}\color{black})/drops(\color{red}{red}\color{black}) shown vs. the default CLIP baseline with manual prompts (i.e. ``a photo of a..."). We show that across visual encoders, both CLIP's internal knowledge and external country-specific LLM knowledge improve classification, especially on Africa and Asia. LLM = \textit{davinci-003}.}
    \label{table:zero_shot}
\end{table*}



==> tables/bacc_soft_prompt.tex <==
 \setlength{\tabcolsep}{4pt}

\begin{table*}[t]

    \begin{center}
        \renewcommand{\arraystretch}{0.9}

    \begin{tabular}{c|c|cc|cc|cc|cc|cc}
        \hline
         && \multicolumn{2}{c|}{\textit{\textbf{Source}}} 
         & \multicolumn{8}{c}{\textit{\textbf{Target}}}  \\
        
         \textbf{Visual Encoder} &
         \textbf{Prompting Method} 
         & \multicolumn{2}{c|}{\textbf{Europe}} 
         & \multicolumn{2}{c}{\textbf{Africa}} 
         & \multicolumn{2}{c}{\textbf{Asia}} 
         & \multicolumn{2}{c}{\textbf{Americas}} 
         & \multicolumn{2}{c}{\textbf{Total}} \\
        
         & & \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c|}{\small $\Delta$} 
         %& \multicolumn{1}{c}{\small OAcc} 
         %& \multicolumn{1}{c|}{\small $\Delta$} 
         & \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c}{\small $\Delta$} 
         %& \multicolumn{1}{c}{\small OAcc} 
         %& \multicolumn{1}{c}{\small $\Delta$} 
         & \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c}{\small $\Delta$} 
        % & \multicolumn{1}{c}{\small OAcc} 
        % & \multicolumn{1}{c}{\small $\Delta$} 
         & \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c}{\small $\Delta$}  
         %& \multicolumn{1}{c}{\small OAcc} 
         %& \multicolumn{1}{c}{\small $\Delta$} 
         & \multicolumn{1}{c}{Acc}
         & \multicolumn{1}{c}{\small $\Delta$} 
         %& \multicolumn{1}{c}{\small OAcc} 
        % & \multicolumn{1}{c}{\small $\Delta$}   
        \\
    
    \hline\hline
    
        \rowcolor{LLGray}\cellcolor{white}  ViT-B/16 &
        
          CoOp \cite{zhou2022learning} 
         % Europe
         &  72.2 & \small - % & \small 73.3 & \scriptsize -
         % Africa
         & 53.9 & \small - % & \small 48.5 & \scriptsize - 
         % Asia
         &  61.5 & \small - % & \small 60.7 & \scriptsize -
         % Americas
         &  68.6 & \small - % & \small 67.8 & \scriptsize -
         % Total
         &  61.7 & \small - % & \small 59.7 & \scriptsize - 
         \\
         
         \rowcolor{LLGray} \cellcolor{white} & CoCoOp \cite{Zhou_2022_CVPR} 
         &  73.2 & \small - %& \small \textbf{74.4} & \scriptsize -
          &  54.3 & \small - %& \small 48.4 & \scriptsize -
         &  61.2 & \small - %& \small 60.6 & \scriptsize -
         & 68.3 & \small - %& \small 67.1 & \scriptsize -
         &  61.4 & \small - %& \small 59.5 & \scriptsize -
         \\
         
         \rowcolor{LLGray} \cellcolor{white} &  KgCoOp ($\lambda$=8) \cite{yao2023visual} 
         & 72.6 & \small - %& \small 73.6 & \scriptsize -
         &  54.1 & \small - %& \small 48.2 & \scriptsize - 
         & 61.5 & \small -% & \small 60.7 & \scriptsize -
         & 68.3 & \small - %& \small 67.0 & \scriptsize -
         &  61.6 & \small - % & \small 59.5 & \scriptsize - 
         \\
        
         \rowcolor{LLGray} \cellcolor{white} &  KgCoOp ($\lambda$=4) \cite{yao2023visual} 
         &  73.1 & \small - %& \small 73.9 & \scriptsize -
         &  54.4 & \small - %& \small 49.5 & \scriptsize - 
         & 62.6 & \small - %& \small 62.1 & \scriptsize - 
         &  68.7 & \small - %& \small 68.0 & \scriptsize -
         &  62.4 & \small - %& \small 60.7 & \scriptsize- 
         \\
         
         & CountryInPrompt Reg 
         &  71.8 & \small \color{red}{-1.4} %& \small 73.4 & \scriptsize \color{red}{-1.0}
         &  56.8 & \small \color{Greenish}{+2.4} % & \small \textbf{52.0} & \scriptsize \color{Greenish}{+2.5} 
         &  63.0 & \small \color{Greenish}{+0.4} %& \small \textbf{63.6} & \scriptsize \color{Greenish}{+1.5} 
         &  69.8 & \small \color{Greenish}{+1.1} %& \small 68.8 & \scriptsize \color{Greenish}{+0.8}
         &  63.5 & \small \color{Greenish}{+1.1} %& \small \textbf{62.3} & \scriptsize \color{Greenish}{+1.6} 
         \\
         
         & CountryLLM Reg 
         &  73.2 & \small \color{black}{0.0} %& \small 73.9 & \scriptsize \color{red}{-0.5}
         &  55.6 & \small \color{Greenish}{+1.2} %& \small 50.6 & \scriptsize \color{Greenish}{+1.1} 
         & 63.0 & \small \color{Greenish}{+0.4}% & \small 62.8 & \scriptsize \color{Greenish}{+0.7}
         &  70.0 & \small \color{Greenish}{+1.3} %& \small \textbf{69.1} & \scriptsize \color{Greenish}{+1.1}
         &  63.2 & \small \color{Greenish}{+0.8} %& \small 61.6 & \scriptsize \color{Greenish}{+0.9} 
         \\
         
         &CountryInPrompt+LLM Reg  
         &  \textbf{73.6} & \small \color{Greenish}{+0.4} %& \small 74.0 & \scriptsize \color{red}{-0.4}
         & \textbf{57.2} & \small \color{Greenish}{+2.8} %& \small 51.9 & \scriptsize \color{Greenish}{+2.4} 
         & \textbf{63.8} & \small \color{Greenish}{+1.2} %& \small 63.4 & \scriptsize \color{Greenish}{+1.3} 
         & \textbf{70.3} & \small \color{Greenish}{+1.6} %& \small 68.8 & \scriptsize \color{Greenish}{+0.8}
         & \textbf{64.0} & \small \color{Greenish}{+1.6} %& \small 62.2 & \scriptsize \color{Greenish}{+1.5} 
         \\
         
    \hline\hline
        
        \rowcolor{LLGray} \cellcolor{white}  RN50 
        
        &  CoOp \cite{zhou2022learning} 
        & 64.6 & \small - %& \small 65.9 & \scriptsize -
        &  45.2 & \small - %& \small 40.3 & \scriptsize - 
        &51.6 & \small - %& \small 51.3 & \scriptsize - 
        &  59.5 & \small - %& \small 58.5 & \scriptsize -
        &  52.2 & \small - %& \small 50.6 & \scriptsize -
        \\
        
        \rowcolor{LLGray} \cellcolor{white} &  CoCoOp \cite{Zhou_2022_CVPR} 
        & 62.9 & \small - %& \small 64.1 & \scriptsize -
        & 44.5 & \small - % & \small 39.1 & \scriptsize - 
        & 51.0 & \small - % & \small 50.3 & \scriptsize - 
        & 58.3 & \small - % & \small 57.7 & \scriptsize -
        &  51.4 & \small - % & \small 49.6 & \scriptsize - 
        \\
        
        \rowcolor{LLGray} \cellcolor{white}  &  KgCoOp ($\lambda$=8) \cite{yao2023visual} 
        &  61.6 & \small - %& \small 64.6 & \scriptsize -
        &  45.2 & \small - %%& \small 41.7 & \scriptsize -
        &  52.6 & \small - %& \small 52.8 & \scriptsize - 
        &  59.6 & \small - %& \small 58.8 & \scriptsize -
        &  52.8 & \small - %& \small 51.8 & \scriptsize -  
        
        \\
        
        \rowcolor{LLGray} \cellcolor{white}  & KgCoOp ($\lambda$=4) \cite{yao2023visual} 
        & 63.5 & \small - %& \small 65.0 & \scriptsize -
        & 46.3 &\small - %& \small 42.2 & \scriptsize - 
        &  53.9 & \small - %& \small 53.4 & \scriptsize - 
        &  \textbf{60.5} & \small - %& \small 59.5 & \scriptsize -
        &  53.9 & \small - % & \small 52.4 & \scriptsize - 
        
        \\
        
        &  CountryInPrompt Reg 
        &  63.5 & \small \color{red}{-1.1}% & \small 64.9 & \scriptsize \color{red}{-1.0}
        &  48.0 & \small \color{Greenish}{+1.7} %& \small 42.9 & \scriptsize \color{Greenish}{+0.7}
        &  53.9 & \small \color{black}{0.0} %& \small 53.9 & \scriptsize \color{Greenish}{+0.5}
        &  60.3 & \small \color{red}{-0.2} %& \small 59.3 & \scriptsize \color{red}{-0.2}
        & 54.3 & \small \color{Greenish}{+0.4} %& \small 52.8 & \scriptsize \color{Greenish}{+0.4}  
        
        \\
        
         &  CountryLLM Reg 
         &  64.5 & \small \color{red}{-0.1} %& \small 65.5 & \scriptsize \color{red}{-0.4}
         & 47.4 & \small \color{Greenish}{+1.1} %& \small 41.7 & \scriptsize \color{red}{-0.5} 
         &  54.2 & \small \color{Greenish}{+0.3}% & \small 53.3 & \scriptsize \color{red}{-0.1}
         &  59.9 & \small \color{red}{-0.6} %& \small 59.2 & \scriptsize  \color{red}{-0.3}
         & 54.3 & \small \color{Greenish}{+0.4} %& \small 52.2 & \scriptsize \color{red}{-0.2} 
         
         \\
         
         & CountryInPrompt+LLM Reg    
         & \textbf{65.5} & \small \color{Greenish}{+0.9} %& \small \textbf{66.8} & \scriptsize \color{Greenish}{+0.9}
         &  \textbf{48.1} & \small \color{Greenish}{+1.8} %& \small \textbf{43.1} & \scriptsize \color{Greenish}{+0.9} 
         & \textbf{54.5} & \small \color{Greenish}{+0.6} %& \small \textbf{54.0} & \scriptsize \color{Greenish}{+0.6}
         &  60.4 & \small \color{red}{-0.1} %& \textbf{59.6} & \small\color{Greenish}{+0.1}
        
        & \textbf{54.8} & \small \color{Greenish}{+0.9} %& \small \textbf{53.0} & \scriptsize \color{Greenish}{+0.6} 
         
         \\

    \hline
    \end{tabular}
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Evaluating country knowledge-regularized soft prompts, top1 balanced accuracy (Acc) on DollarStreet.} We emphasize that our regularization aims to improve \textbf{target} performance on unseen geographies, rather than source. We compare regularizing prompts with country names (CountryInPrompt), country-specific LLM knowledge (CountryLLM), and both (CountryInPrompt+LLM), with gains(\color{Greenish}{green}\color{black})/drops(\color{red}{red}\color{black}) shown vs. the \textit{best} of various soft prompt baselines. Our CountryInPrompt+LLM achieves notable gains in target, especially on Africa. We use regularization weight $\lambda$=4, so we compare to KgCoOp at $\lambda$=8 (default) and $\lambda$=4. Each method uses 16 shots \& context length 4.}
    \label{table:soft_prompt}
\end{table*}

==> tables/bacc_zeroshot.tex <==
 \setlength{\tabcolsep}{4pt}

\begin{table*}[t]

    \begin{center}
    \renewcommand{\arraystretch}{0.9}

    \begin{tabular}{c|c|cc|cc|cc|cc|cc}
        \hline
        \textbf{Visual Encoder} & \textbf{Prompting Method} & \multicolumn{2}{c}
        {\textbf{ Europe}} & \multicolumn{2}{c}{\textbf{Africa}} &\multicolumn{2}{c}{\textbf{Asia}} & \multicolumn{2}{c}{\textbf{Americas}} & \multicolumn{2}{c}{\textbf{Total}} \\
         & 
         &  \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c}{$\Delta$} 
         %&  \multicolumn{1}{c}{\small OAcc} 
         %& \multicolumn{1}{c}{\small $\Delta$} 
         &  \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c}{ $\Delta$} 
         %&  \multicolumn{1}{c}{\small OAcc} 
         %& \multicolumn{1}{c}{\small $\Delta$} 
         & \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c}{ $\Delta$} 
         %&  \multicolumn{1}{c}{\small OAcc}
         %& \multicolumn{1}{c}{\small $\Delta$}
         &  \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c}{$\Delta$} 
         %&  \multicolumn{1}{c}{\small OAcc} 
         %& \multicolumn{1}{c}{\small $\Delta$}
         & \multicolumn{1}{c}{Acc} 
         & \multicolumn{1}{c}{$\Delta$} 
        % &  \multicolumn{1}{c}{\small OAcc} 
        % & \multicolumn{1}{c}{\small $\Delta$}
         
         \\
    \hline\hline \rowcolor{LLGray}
        \cellcolor{white} ViT-B/32  
        &  Zero-Shot CLIP \cite{radford2021learning} 
        & 59.1 & \small - 
        %& \small 56.3 & \scriptsize - 
        &  43.7 & \small - 
        %& \small 38.3 & \scriptsize - 
        &  50.8 & \small - 
        %& \small 47.4 & \scriptsize - 
        &  \textbf{55.3} & \small - 
        %& \small 53.1 & \scriptsize - 

        &  51.7 & \small -
        %& \small 48.3 & \scriptsize -
        
        \\
        
         \rowcolor{LLGray}
        \small \cellcolor{white} & GeneralLLM \cite{menon2022visual}
         & 57.3 & \small \color{red}{-1.8} 
         %& \small 55.4 & \scriptsize \color{red}{-0.9} 
         &44.3 & \small \color{Greenish}{+0.6} 
         %& \small 38.4 & \scriptsize \color{Greenish}{+0.1} 
         &  50.9 & \small \color{Greenish}{+0.1} 
         %& \small 48.2 & \scriptsize \color{Greenish}{+0.8} 
         &  54.6 & \small \color{red}{-0.7} 
         %& \small 52.2 & \scriptsize \color{red}{-0.9} 

         &  51.4 & \small \color{red}{-0.3}
         %& \small 48.4 & \scriptsize \color{Greenish}{+0.1} 
         \\

         &  CountryInPrompt 

         & 57.5 & \small \color{red}{-1.6} 
         %& \small 55.2 & \scriptsize \color{red}{-1.1} 
         & 45.2 & \small \color{Greenish}{+1.5} 
         %& \small 41.0 & \scriptsize \color{Greenish}{+2.7} 
         &  51.9 & \small \color{Greenish}{+1.1} 
         %& \small 49.7 & \scriptsize \color{Greenish}{+2.3} 
         &  55.0 & \small \color{red}{-0.3} 
        % & \small 52.3 & \scriptsize \color{red}{-0.8} 

         &  52.1 & \small \color{Greenish}{+0.4}
         %& \small 49.5 & \scriptsize \color{Greenish}{+1.2} 
         \\
         
         &  CountryLLM 
         &  59.4 & \small \color{Greenish}{+0.3} 
         %& \small \textbf{57.5} & \scriptsize \color{Greenish}{+1.2} 
         &  45.2 & \small \color{Greenish}{+1.5} 
         %& \small 40.7 & \scriptsize \color{Greenish}{+2.4} 
         & 52.1 & \small \color{Greenish}{+1.3} 
         %& \small 49.6 & \scriptsize \color{Greenish}{+2.2} 
         & \textbf{55.3} & \small \color{black}{0.0} 
         %& \small \textbf{53.4} & \scriptsize \color{Greenish}{+0.3} 

         &  52.6 & \small \color{Greenish}{+0.9}
        % & \small 50.0 & \scriptsize \color{Greenish}{+1.7} 
        \\
         

         
         & CountryInPrompt+LLM  
          &  \textbf{60.8} & \small \color{Greenish}{+1.7}
         %& \small \textbf{57.5} & \scriptsize \color{Greenish}{+1.2} 
         &  \textbf{45.3} & \small \color{Greenish}{+1.6} 
         %& \small \textbf{41.3} & \scriptsize \color{Greenish}{+3.0} 
         & \textbf{52.2} & \small \color{Greenish}{+1.4}
         %& \small \textbf{50.1} & \scriptsize \color{Greenish}{+2.7}
         &  55.0 & \small \color{red}{-0.3} 
         %& \small 52.9 & \scriptsize \color{red}{-0.2} 

         &  \textbf{52.8} & \small \color{Greenish}{+1.1}
        % & \small \textbf{50.3} & \scriptsize \color{Greenish}{+2.0}
        \\
         
    \hline\hline \rowcolor{LLGray}
         \cellcolor{white}ViT-B/16  &  Zero-Shot CLIP \cite{radford2021learning}  
        & 64.3 & \small - 
       %& \small 61.5 & \scriptsize - 
       &  46.9 & \small - 
       %& \small 42.9 & \scriptsize - 
       &  53.9 & \small - 
       %& \small 52.7 & \scriptsize - 
       &  \textbf{60.1} & \small - 
       %& \small 58.0 & \scriptsize - 
       &  55.5 & \small - 
       %& \small 53.4 & \scriptsize - 
       \\
       
         \rowcolor{LLGray}
        \cellcolor{white} & GeneralLLM \cite{menon2022visual} 
          &  64.2 & \small \color{red}{-0.1} 
         %& \small 61.4 & \scriptsize \color{red}{-0.1} 
         &  48.8 & \small \color{Greenish}{+1.9} 
         %& \small 44.9 & \scriptsize \color{Greenish}{+2.0} 
         & \textbf{56.0} & \small \color{Greenish}{+2.1} 
        % & \small 55.0 & \scriptsize \color{Greenish}{+2.3} 
         &  58.5 & \small \color{red}{-1.6} 
         %& \small 56.9 & \scriptsize \color{red}{-1.1} 

         &  56.8 & \small \color{Greenish}{+1.3}
        % & \small 54.6 & \scriptsize \color{Greenish}{+1.2} 
        \\

         
         & CountryInPrompt 
         &  63.9 & \small \color{red}{-0.4} 
         %& \small 61.5 & \scriptsize \color{black}{0.0} 
         &  49.6 & \small \color{Greenish}{+2.7} 
         %& \small 46.2 & \scriptsize \color{Greenish}{+3.3} 
         &  55.7 & \small \color{Greenish}{+1.8} 
        % & \small 54.8 & \scriptsize \color{Greenish}{+2.1} 
         &  59.3 & \small \color{red}{-0.8} 
         %& \small 57.1 & \scriptsize \color{red}{-0.9} 

         & 56.6 & \small \color{Greenish}{+1.1}
         %& \small 54.8 & \scriptsize \color{Greenish}{+1.4}
         \\

         &  CountryLLM  
         &  65.2 & \small \color{Greenish}{+0.9} 
        % & \small \textbf{62.9} & \scriptsize \color{Greenish}{+1.4} 
         &  49.6 & \small \color{Greenish}{+2.7} 
         %& \small 45.4 & \scriptsize \color{Greenish}{+2.5} 
         & 55.6 & \small \color{Greenish}{+1.7} 
         %& \small 54.9 & \scriptsize \color{Greenish}{+2.2} 
         & 59.7 & \small \color{red}{-0.4} 
         %& \small \textbf{58.4} & \scriptsize \color{Greenish}{+0.4} 

         &  57.0 & \small \color{Greenish}{+1.5}
         %& \small 55.1 & \scriptsize \color{Greenish}{+1.7} 
         \\
         
         &  CountryInPrompt+LLM 
         &  \textbf{65.5} & \small \color{Greenish}{+1.2} 
         %& \small 62.6 & \scriptsize \color{Greenish}{+1.1} 
         & \textbf{50.8} & \small \color{Greenish}{+3.9} 
         %& \small \textbf{47.1} & \scriptsize \color{Greenish}{+4.2} 
         & \textbf{56.0} & \small \color{Greenish}{+2.1} 
         %& \small \textbf{55.7} & \scriptsize \color{Greenish}{+3.0} 
         &  59.7 & \small \color{red}{-0.4} 
        % & \small 58.2 & \scriptsize \color{Greenish}{+0.2} 
         &  \textbf{57.4} & \small \color{Greenish}{+1.9}
         %& \small \textbf{55.8} & \scriptsize \color{Greenish}{+2.4}
         \\
    \hline
    \hline
    \rowcolor{LLGray}
         \cellcolor{white} RN50 
        &  Zero-Shot CLIP \cite{radford2021learning} 
        &  53.0 & \small - 
        %& \small 51.8 & \scriptsize - 
        &  38.0 & \small - 
       % & \small 34.4 &  \scriptsize - 
        &  44.4 & \small - 
       % & \small 44.0 & \scriptsize - 
        &  49.8 & \small - 
       % & \small 47.3 & \scriptsize - 

        &  45.7 & \small -
       % & \small 44.2 & \scriptsize - 
       \\
        

         \rowcolor{LLGray}
        \small \cellcolor{white} &  GeneralLLM \cite{menon2022visual}
         &  55.5 & \small \color{Greenish}{+2.5} 
        % & \small 53.2 & \scriptsize \color{Greenish}{+1.4} 
         & 40.9 & \small \color{Greenish}{+2.9} 
         %& \small 36.0 & \scriptsize \color{Greenish}{+1.6} 
         & 46.9 & \small \color{Greenish}{+2.5} 
         %& \small 45.0 & \scriptsize \color{Greenish}{+1.0} 
         &  50.3 & \small \color{Greenish}{+0.4} 
         %& \small 48.3 & \scriptsize \color{Greenish}{+1.0}

         &  47.9 & \small \color{Greenish}{+2.2}
         %& \small 45.4 & \scriptsize \color{Greenish}{+1.2}   
         \\
         

         
         &  CountryInPrompt 

         & 54.5 & \small \color{Greenish}{+1.5} 
         %& \small 52.2 & \scriptsize \color{Greenish}{+0.4} 
         &  \textbf{43.4} & \small \color{Greenish}{+5.4} 
         %& \small 38.7 & \scriptsize \color{Greenish}{+4.3} 
         &  47.0 & \small \color{Greenish}{+2.6} 
         %& \small 45.4 & \scriptsize \color{Greenish}{+1.4}
         &  50.8 & \small \color{Greenish}{+1.0} 
         %& \small 48.5 & \scriptsize \color{Greenish}{+1.2} 

         &  48.4 & \small \color{Greenish}{+2.7}
        % & \small 45.9 & \scriptsize \color{Greenish}{+1.7}   
        \\

         &  CountryLLM 
         &  56.2 & \small \color{Greenish}{+3.2}
         %& \small 54.1 & \scriptsize \color{Greenish}{+2.3} 
         &  41.1 & \small \color{Greenish}{+3.1} 
         %& \small 36.9 & \scriptsize \color{Greenish}{+2.5} 
         &   47.3 & \small \color{Greenish}{+2.9} 
         %& \small 45.7 & \scriptsize \color{Greenish}{+1.7} 
         & 50.4 & \small \color{Greenish}{+0.6} 
         %& \small 48.7 & \scriptsize \color{Greenish}{+1.4} 

         &  48.3 & \small \color{Greenish}{+2.6}
        % & \small 46.1 & \scriptsize \color{Greenish}{+1.9} 
        \\
         
         &  CountryInPrompt+LLM 
         & \textbf{56.4} & \small \color{Greenish}{+3.4}
         %& \small \textbf{54.7} & \scriptsize \color{Greenish}{+2.9} 
         &  43.0 & \small \color{Greenish}{+5.0} 
         %& \small \textbf{38.9} & \scriptsize \color{Greenish}{+4.5}
         &  \textbf{48.0} & \small \color{Greenish}{+3.6} 
         %& \small \textbf{47.1} & \scriptsize \color{Greenish}{+3.1} 
         &  \textbf{50.9} & \small \color{Greenish}{+1.1} 
         %& \small \textbf{49.6}  & \scriptsize \color{Greenish}{+2.3} 

         & \textbf{49.1} & \small \color{Greenish}{+3.4}
         %& \small \textbf{47.3} & \scriptsize \color{Greenish}{+3.1}
         \\ 
    \hline
    \end{tabular}
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Zero-shot CLIP with descriptive knowledge prompts, top1 balanced accuracy (Acc) on DollarStreet.} We test the methodology from \cite{menon2022visual}, our country-specific LLM probing (CountryLLM), adding country names to prompts (CountryInPrompt), and both country strategies combined (CountryInPrompt+LLM), with gains(\color{Greenish}{green}\color{black})/drops(\color{red}{red}\color{black}) shown vs. the default CLIP baseline with manual prompts (i.e. ``a photo of a..."). We show that across visual encoders, both CLIP's internal knowledge and external country-specific LLM knowledge improve classification, especially on Africa and Asia. LLM = \textit{davinci-003}.}
    \label{table:zero_shot}
\end{table*}



==> tables/ex_prompts_for_reg.tex <==
\begin{table*}[t]

    \begin{center}
    \begin{tabular}{c|c|c|c}
        \textbf{Prompting Method} & \textbf{Text Embedding} & \textbf{Prompt}   \\
    \hline
        \small Default &  \small Template & \small ``a photo of a $<$object$>$" \\
    \hline 
        \small InCountry &  \small & \small ``a photo of a $<$object$>$ in $<$country$>$ " \\ 
    \hline 
        \small CountryLLM & \small Template & \small ``a photo of a $<$object$>$ which (is/has/etc.) $<$descriptor$>$" \\

    \hline 
        \small InCountry + CountryLLM &  \small Template & \small ``a photo of a $<$object$>$ in $<$country$>$ which (is/has/etc.) $<$descriptor$>$"\\
    \hline 
    \end{tabular}
    \end{center}
    \caption{Prompt forms of experimentation. }
    \label{table:ex_prompt}
\end{table*}

==> tables/sina_geonet/soft_prompt_table.tex <==
 \setlength{\tabcolsep}{4.0pt}

\begin{table*}[t]

    \begin{center}
    \begin{tabular}{c|c|c|c|ccc|c}
        \hline
        && \multicolumn{2}{c|}{\textit{\textbf{Source}}} & \multicolumn{2}{c}{\textit{\textbf{Target}}}\\
        \textbf{Encoder} & \textbf{Prompting Method} & \multicolumn{2}{c|}{\textbf{USA}} &\multicolumn{2}{c}{\textbf{Asia}} \\
         & &  \multicolumn{1}{c}{overal Acc} & \multicolumn{1}{c|}{$\Delta$} &  \multicolumn{1}{c}{macro-acc}& \multicolumn{1}{c}{overal Acc}& \multicolumn{1}{c}{macro-f1} & \multicolumn{1}{c}{$\Delta$} \\
    \hline\hline
            ViT-B/16 
        & CoOp \cite{zhou2022learning} & 59.87&-& 51.20 &51.70&48.30& -   \\ \hline
         & KgCoOp (w=4) \cite{yao2023visual} & 60.03 & -&52.47&53.23& 50.00  &-  \\
         & ``In Country (w=4)'' Reg & 59.23&- &53.73& 53.97& 50.70 &-  \\
         & LLM Reg (w=4) & 60.20& - &52.93 &53.57& 50.30 & - \\
         & ``In Country''+LLM Reg (w=4) &  59.40&- & 53.50&53.83&50.40&-  \\ \hline
        & KgCoOp (w=8) \cite{yao2023visual} &59.40 &- &  52.57& 53.50& 50.30&- \\
         & ``In Country (w=8)'' Reg & 58.70&- &53.47&53.77 & 50.50&-  \\
         & LLM Reg (w=8) & 59.93& - &53.13& 54.03&  50.57 & - \\
         & ``In Country''+LLM Reg (w=8) & 58.93&- & \textbf{53.93}& 54.23& 50.93&-  \\
        \hline
         & $L_{contrastive}$ + src KD (w=8) &0.0&-& 53.67 &\textbf{54.53}& \textbf{51.20}&-\\
         & $L_{contrastive}$ + tgt KD (w=8) &0.0&-& 53.37 &54.23 & 50.87 &-\\
         & $L_{contrastive}$ + src KD +in-country (w=8) &0.0&-& 52.90 & 53.73&  50.50 &-\\
    \hline\hline
        ResNet50 
        & CoOp \cite{zhou2022learning} & 52.70&- &45.57 &  45.87&  42.37 &-  \\ \hline
         & KgCoOp (w=4) \cite{yao2023visual} &  53.23& - &46.83  &47.70 & 44.50& -  \\
         & ``In Country'' Reg (w=4) &  52.10& - & 47.67 & 48.00 &  44.63 & -  \\
         & LLM Reg (w=4) & 53.10&- &47.03  &47.83 &  44.47 & -  \\
         & ``In Country''+LLM Reg (w=4) &52.87& -  & \textbf{48.27} &\textbf{ 48.53} & \textbf{45.20} & -  \\ \hline
        & KgCoOp (w=8) \cite{yao2023visual} & 52.70& - & 46.87 & 47.90 & 44.80& -\\
         & ``In Country'' Reg (w=8) & 51.53& - & 47.63 & 48.00 &  44.57 & -  \\
         & LLM Reg (w=8) & 52.83&- &47.43  &48.43&  45.07 & -  \\
         & ``In Country''+LLM Reg (w=8) & 52.13& -  &48.30 & 48.63&  45.37 & -  \\

    \hline
    \end{tabular}
    \end{center}
    \caption{\textbf{Soft Prompt on GeoNet. Average per class accuracy with top 10 country ensemble}}
    \label{table:sof245t_prompt}
\end{table*}

==> tables/zero_shot_results_geonet.tex <==
 \setlength{\tabcolsep}{4.0pt}

\begin{table}[t]

    \begin{center}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Encoder} & \textbf{Prompting Method} & \multicolumn{2}{c}{\textbf{Europe}} &\multicolumn{2}{c}{\textbf{America}} & \multicolumn{2}{c}   {\textbf{Asia}} & \multicolumn{2}{c}{\textbf{Africa}} & \multicolumn{2}{c}{\textbf{Total}} \\
         & &  \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{$\Delta$} &  \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{$\Delta$} &  \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{$\Delta$} &  \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{$\Delta$} &  \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{$\Delta$}  \\
    \hline
        ResNet50  & Zero-Shot CLIP \cite{radford2021learning} \\
         & GeneralLLM \cite{menon2022visual} \\
         & CountryLLM  \\
         & ``In Country"  \\
         & ``In Country"+CountryLLM \\
         & ``In Country"+CountryLLM (ChatGPT) \\
    \hline
        ViT-B/32 & Zero-Shot CLIP \cite{radford2021learning} \\
         & GeneralLLM \cite{menon2022visual} \\
         & CountryLLM  \\
         & ``In Country"  \\
         & ``In Country"+CountryLLM \\
         & ``In Country"+CountryLLM (ChatGPT) \\
    \hline
    \end{tabular}
    \end{center}
    \caption{\textbf{Zero-Shot Knowlege Integration DollarStreet} Gauging the geographical robustness of common m=16; LLM = ? . We are the first to explore these country-specific variants.}
    \label{table:zero_shot}
\end{table}
